Active Distribution Learning from Indirect Samples

This paper studies the problem of {\em learning} the probability distribution $P_X$ of a discrete random variable $X$ using indirect and sequential samples. At each time step, we choose one of the possible $K$ functions, $g_1, \ldots, g_K$ and observe the corresponding sample $g_i(X)$. The goal is to estimate the probability distribution of $X$ by using a minimum number of such sequential samples. This problem has several real-world applications including inference under non-precise information and privacy-preserving statistical estimation. We establish necessary and sufficient conditions on the functions $g_1, \ldots, g_K$ under which asymptotically consistent estimation is possible. We also derive lower bounds on the estimation error as a function of total samples and show that it is order-wise achievable. Leveraging these results, we propose an iterative algorithm that i) chooses the function to observe at each step based on past observations; and ii) combines the obtained samples to estimate $p_X$. The performance of this algorithm is investigated numerically under various scenarios, and shown to outperform baseline approaches.

==> applications.tex <==

\section{Possible Applications}
\label{sec:app}

\subsection{Diagnosing System Failure}
The random variable $X$ represents an unknown cause of the failure of a system. To determine the cause, we can run $K$ different diagnostic tests and measure their result. Our objective is to determine as soon as possible the treatment $g_{i^*}(X)$ that is most effective. The effectiveness of a treatment may not be binary; it can be partially effective. \color{red} One objective could be to understand the cause of failure.. why is $X$ a distribution? \color{black}

\subsection{Estimating service time distribution}
launch replicas (functions..), observe response time which is a function of service time distribution and number of replicas... Estimating service time distribution will help design better policies..

\subsection{Portfolio choice problem}
Maybe not relevant in this setting

\subsection{Ad placement / social networks}
Ad placement companies can present an ad to a user community, the click through rates corresponding to different ads are a function of the nature of user community. (nature could be something like age distribution, salaries etc). Objective is to try to understand this hidden nature as quickly as possible. 

\subsection{Estimating probability distribution of bacterial concentrations}
testing different samples of food (arms of bandit) on a certain metric (observations), metric is a function of bacterial concentrations,  trying to estimate probability distributions of these bacterial concentrations. 

\subsection{Gene expression data}
\color{red} not sure \color{black}



\TODO{Think of more applications}



==> related_work.tex <==
\section{Related Prior Work}

Learning the distribution of a random variable $X$ from a set of empirical samples is a well-studied research problem \cite{valiant1984theory, kearns1994learnability} in theoretical computer science. Many works are interested in finding the min-max or worst case loss \cite{kamath2015learning} for various loss functions such as L2-loss and Kullback-Liebler (KL) divergence. Unlike most works in distribution learning theory, where samples of $X$ are given, we only have access to samples of functions $g_i(X)$. In this framework, we seek to minimize the simpler expected L2-loss.

Inferring a hidden random variable from indirect samples is related to many works in estimation theory \cite{kay1993fundamentals}, where objective is to estimate a set of parameters $\theta$ using observations $y_1, y_2 , \dots y_n$ that follow a model $p(Y|\theta)$. In our problem, the hidden variable $X$ is analogous to the parameter $\theta$ while samples $g_i(X_t)$ correspond to the observations $y_1, y_2 , \dots y_n$. We use maximum-likelihood estimation to combine samples, and use the Cramer-Rao bound  \cite{rao1945information, cramer1946mathematical} to obtain a lower bound on the variance of our estimator. 

However a key difference is that unlike typical parameter estimation problems, we can choose the arm $i$ that is pulled in each slot to obtain sample $g_i(X)$. This aspect is closely related to the  multi-arm bandit framework \cite{bubeck2012regret} in reinforcement learning. Since the rewards $g_1(X), g_2(X), \ldots g_K(X)$ depend on a common source of randomness, pulling one arm can provide us information about the distribution of $X$, which in turn can help estimate the expected reward from other arms. In other words, unlike the classical multi-arm bandit problem, the arms are correlated through the hidden variable $X$. 

